VEXP: A Low-Cost RISC-V ISA Extension for Accelerated Softmax Computation in Transformers

While Transformers are dominated by Floating-Point (FP) Matrix-Multiplications, their aggressive acceleration through dedicated hardware or many-core programmable systems has shifted the performance bottleneck to non-linear functions like Softmax. Accelerating Softmax is challenging due to its non-pointwise, non-linear nature, with exponentiation as the most demanding step. To address this, we design a custom arithmetic block for Bfloat16 exponentiation leveraging a novel approximation algorithm based on Schraudolph's method, and we integrate it into the Floating-Point Unit (FPU) of the RISC-V cores of a compute cluster, through custom Instruction Set Architecture (ISA) extensions, with a negligible area overhead of 1\%. By optimizing the software kernels to leverage the extension, we execute Softmax with 162.7$\times$ less latency and 74.3$\times$ less energy compared to the baseline cluster, achieving an 8.2$\times$ performance improvement and 4.1$\times$ higher energy efficiency for the FlashAttention-2 kernel in GPT-2 configuration. Moreover, the proposed approach enables a multi-cluster system to efficiently execute end-to-end inference of pre-trained Transformer models, such as GPT-2, GPT-3 and ViT, achieving up to 5.8$\times$ and 3.6$\times$ reduction in latency and energy consumption, respectively, without requiring re-training and with negligible accuracy loss.

==> TEXT/01_Introduction.tex <==
\section{Introduction}

Transformer-based models~\cite{vaswani_attention_2017}, such as the GPT family~\cite{guo_gptqt_2024} and the LLaMa family~\cite{touvron_llama_2023}, have emerged as a cornerstone of machine learning, demonstrating state-of-the-art performance in diverse domains, including natural language processing (NLP), computer vision, and audio processing. These models leverage pre-trained representations on large-scale unlabeled datasets, enabling remarkable accuracy improvements in fine-tuned downstream tasks such as sentence classification and question answering. At the core of their success is the Transformer architecture \cite{vaswani_attention_2017}, which utilizes the self-attention mechanism to model complex relationships within input sequences. 

However, the deployment of Transformer-based models presents significant computational demands and challenges in meeting energy constraints towards the edge. In encoders and the prefill stage of decoders, the computational complexity of the attention mechanism scales quadratically with the input sequence length, resulting in substantial memory and computational overhead. While many architectures incorporate \gls{gemm} acceleration to mitigate computational burden, performance bottlenecks are increasingly shifting toward non-linear operations, particularly the Softmax function within the attention layers.
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{01Image/gpt_3_baseline.pdf}
\caption{Runtime breakdown for GPT-3 on a RISC-V multi-cluster platform~\cite{potocnik_optimizing_2024}. For each sequence length, the left bar shows unoptimized \gls{gemm} results, while the right bar reflects optimized \gls{gemm} results.}
\label{image:introduction}
\end{figure}
The Softmax function, which transforms attention scores into pseudo-probabilities, plays a central role in the attention mechanism. However, it presents several challenges due to its non-linear, non-pointwise nature and reliance on a transcendental function, namely exponentiation. The low arithmetic intensity of Softmax constrains parallelism and processing efficiency, a limitation that becomes more pronounced as \gls{gemm} latency decreases with acceleration. The runtime breakdown for BERT on Volta GPU from Steven et al.~\cite{stevens_softermax_2021} shows Softmax contributes more than 30\% for long sequences. Moreover, as shown in \autoref{image:introduction}, deployment of GPT3-XL on the RISC-V multi-cluster platform \cite{potocnik_optimizing_2024} reveals that Softmax contributes to 30\% of the runtime prior to \gls{gemm} operator acceleration, and 70\% afterwards for sequence length of 2048.
% , which processes 16 attention heads with a hidden size of 2048.

%Given its role in ensuring model numerical stability, Softmax computation demands high precision, especially in large-scale scenarios or when operating with low-precision data. 


Overcoming these challenges requires innovative solutions that optimize the Softmax function while maintaining the accuracy of Transformer-based models. Existing software-level optimizations~\cite{kim_i-bert_2021} often fall short of delivering the accuracy, performance and efficiency improvements necessary for large-scale or low-power deployments. While hardware accelerators are effective in enhancing performance and energy efficiency, they often lack flexibility due to their reliance on custom and approximate arithmetic blocks. Moreover, achieving accuracy parity often necessitates retraining~\cite{stevens_softermax_2021}~\cite{islamoglu_ita_2023}—a technique that is impractical and undesirable for \glspl{llm}. In contrast, the open and extensible nature of RISC-V, combined with its growing adoption in domain-specific accelerators, offers an ideal foundation for addressing these limitations. By leveraging custom instruction extensions, RISC-V enables efficient and tailored acceleration of computationally intensive operations like Softmax at a very low cost, providing a path to significant performance and energy gains without compromising programmability and model accuracy. 

In this work, we identify the exponential function as the primary computational bottleneck in Softmax computation. Therefore, we propose a novel method to accelerate Softmax for a RISC-V-based system with low hardware overhead. The contributions of this paper are:
\begin{itemize}
% \item We develop a hardware-friendly approximation of the exponential function using the optimized Schraudolph algorithm by Belano et al.\cite{belano_flexible_2024}, implemented with BF16 precision and integrate this unit as an ISA extension to the FPU of Snitch core, with minimal area (1.0\%) and power (1.8\%) overhead.

 %\item By performing HW/SW co-design of Softmax kernel with our new EXP instruction, we achieve a 162.7$\times$ reduction in latency and 74.3$\times$ improvement in energy consumption compared to a software baseline. We integrate our fully optimized Softmax kernel into FlashAttention-2, showing 8.2$\times$ performance and 4.1$\times$ energy efficiency improvement.

 %\item We also demonstrate the scalability of our solution to larger computing systems, enabling broader deployment potential. These optimizations lead to end-to-end performance improvements for Transformer-based models such as GPT-2, GPT-3, and Vision Transformer (ViT), yielding up to 5.8$\times$ and 3.6$\times$ reductions in latency and energy consumption, respectively compared with implementations without Softmax optimizations. Notably, these gains are achieved without retraining and with an accuracy loss of less than 0.1\%.

\item We develop a custom arithmetic block for accelerating the exponential function on \glsentrylong{bf16} data, integrate it in the \gls{fpu} of programmable RISC-V processors of an octa-core compute cluster, and extend their \gls{isa} with a custom EXP instruction;

\item We implement the cluster using GlobalFoundries \qty[detect-all=true]{12}{\nano\meter} technology down to silicon-ready design and demonstrate that our solution incurs only a 1.0\% area overhead at the cluster level and a negligible power overhead of 1.8\% on workloads that do not exploit EXP while the energy required to execute one exponential operation is reduced by two orders of magnitude;

\item By exploiting the proposed \gls{isa} extension, we optimize the execution of Softmax in software, demonstrating 162.7$\times$ latency reduction and 74.3$\times$ less energy consumption compared to a non-optimized kernel on the baseline cluster. Moreover, we integrate our fully optimized Softmax kernel into FlashAttention-2, showing 8.2$\times$ performance and 4.1$\times$ energy efficiency improvements;

\item We scale up the proposed cluster to a 16-cluster system to evaluate the acceleration capabilities of our solutions on end-to-end execution of pre-trained, un-tuned transformers. We benchmark models such as GPT-2, GPT-3, and Vision Transformers (ViT), achieving up to 5.8$\times$ latency reduction and up to 3.6$\times$ less energy consumption compared to a baseline system without the proposed optimizations. Notably, these gains are achieved without re-training and with an accuracy loss of less than 0.1\%.

\end{itemize}

==> TEXT/04_HW_SW_Optimizations.tex <==
\section{Methods}

\subsection{EXP Custom Arithmetic Block}
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{01Image/exps&correction.drawio.pdf}
\caption{Block diagram of (a) the extended \gls{fpu}, (b) the EXP block, (c) the EXP lane, (d) the $exps(x)$ stage, and (e) the $P(x)$ stage.} 
\label{datapath}
\end{figure}

%Based on EXP datapath from {\autoref{datapath}}.EXP, this work proposes a custom combinatorial arithmetic block designed to efficiently compute the exponential function. 

\autoref{datapath}c shows the proposed arithmetic block to efficiently compute the exponential function on Bfloat16 data. This block is structured around the algorithm introduced in \autoref{subsec:exp_approximation} and consists of two cascaded stages: \textbf{$exps(x)$}, which implements the Schraudolph's method in hardware, and the subsequent \textbf{$P(x)$}, which performs the mantissa correction for improved precision. 


At the input of the \textbf{$exps(x)$} stage (shown in \autoref{datapath}d), the data in Bfloat16 format is decomposed into its sign, exponent, and mantissa bits, with the implicit leading 1 appended to the latter. Next, the mantissa is multiplied by the precomputed constant ($\log_2 e$), and the result of this multiplication is then shifted 
by an amount equal to the difference between the exponent of the argument and the maximum exponent after which the exponential function is guaranteed to overflow (133 in the case of BFloat16 numbers).
%based on the input exponent, where the amount of change is calculated by the bias of the format and the field width of the exponent. 
Then, the first 15 bits of the shifted mantissa are selected and appropriately rounded to maintain precision, and finally, if no overflow occurs, the result is obtained by appending a leading zero (the sign bit of the result) to the rounded mantissa and adding the bias to the new exponent. Alternatively, if an overflow is detected, the output is assigned to $\infty$ or $0$, depending on whether the argument is positive or negative.

The second stage of the exponential computation, \textbf{$P(x)$}, corrects the mantissa component of the approximation. First, the MSB of the mantissa determines whether the input falls within \([0, 0.5)\) or \([0.5, 1)\), selecting the appropriate polynomial branch. In the first branch, corresponding to \(x \in [0, 0.5)\), the polynomial \(\alpha x (x + \gamma_1)\) is evaluated directly using fixed-point arithmetic. For \(x \in [0.5, 1)\), the computation proceeds with \(\mathrm{not}(\beta\, \mathrm{not}(x) \cdot (x + \gamma_2))\), where the bitwise complement operation simplifies the evaluation of \(1 - x\). 

Finally, the output of the EXP block is obtained by concatenating the corrected mantissa from the \textbf{$P(x)$} stage with the sign and exponent fields from the \textbf{$exps(x)$} stage.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Snitch \gls{isa} Extension and $\mu$Architecture}

% here we need to provide details and insights on the integration of the Arithmetic block into the \gls{fpu} of the snitch core. 
% Moreover, we need to explain how this unit can be enabled in SW, and that's through custom instruction in the ISA  (we should provide a name to this instruction. For example, pv.mlexp or something better)...here the details should focus on the encoding of instructions, which are the inputs/outputs of the instructions and so on...
% Then, we need to provide some details on how this instruction can be used in your C code..

% \subsubsection{Integration of the EXP Block into the CVFPU Framework}
To exploit the fast exponentiation of Bfloat16 data enabled by the designed EXP block, we integrate it into the \gls{fpu} of the Snitch core, as shown in \autoref{datapath}a) and b). The integration process begins by embedding the EXP block into the CVFPU framework \cite{bertaccini_minifloat-nn_2022}. CVFPU is a highly modular framework designed to support a wide array of floating-point operations, with its functionalities organized into specific modules such as \texttt{FMA} (fused multiply-add), \texttt{DIVSQRT} (division and square root), \texttt{COMP} (comparison), \texttt{CAST} (conversion), and \texttt{SDOTP} (dot product). The EXP block is introduced as a dedicated module within this framework, specifically for BF16 exponentiation.

To support the processing element's capability for double-precision instructions, the Snitch floating-point register file is designed with 64-bit entries, which allows the packing of four BF16 values. The \gls{fpu} interface accommodates up to three 64-bit input operands and produces one 64-bit output per cycle. As illustrated in \autoref{datapath}b, the EXP block incorporates four parallel exponential computation lanes within a single block, enabling 4-way \gls{simd} computation. Each EXP lane is equipped with one level of pipeline registers to streamline processing.

% \textbf{\gls{isa} Extensions}: 
To enable the new functionality, two custom instructions are added to the Snitch \gls{isa}: \texttt{FEXP} for scalar computations and \texttt{VFEXP} for vectorized exponential computations. As shown in \autoref{tab:riscv_encodings}, the instruction formats use \texttt{rd} (destination register) and \texttt{rs1} (source register) as 5-bit fields to address the \gls{fpu}’s 32$\times$64 register file, with the most significant bit of the entire instruction distinguishing between scalar and \gls{simd} vector operations. The Snitch core’s decoder and \gls{fpu} subsystem were updated to support these instructions and seamlessly activate the EXP block in \gls{fpu}.

\begin{table}[t]
\centering
\caption{RISC-V Encodings for FEXP and VFEXP}
\label{tab:riscv_encodings}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lc}
\toprule
\textbf{Format}        & \textbf{Encoding (32-bit)}        \\ 
\midrule
\texttt{\textbf{FEXP} \ rd, rs1}  & \texttt{001111100000\{rs1\}000\{rd\}1010011} \\ 
\texttt{\textbf{VFEXP} rd, rs1} & \texttt{101111100000\{rs1\}000\{rd\}1010011} \\ 
\bottomrule
\end{tabular}
\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% 
% starting from the baseline implementation presented in Section...
% we optimize the softmax function to exploit the underlying ISA, including the design instruction
% The softmax consists of three steps: max, exp, normalization
% since the max is needed for exp and it has to be looped over each element of each row of the QKt resulting matrix, we build the loop with FREP instruction; since we target BF16 and the core's datapath is 64-bit, we also exploit the VFMAX present in the ISA to improve the computation vs loads cost (ie with a load of 64-bit data we can perform 4 \gls{simd} operation). To streamline the loads and keep the datapath busy we exploit the SSRs
% The results are then output to the EXP part, where we use mainly the same kernel's structure with FREP and SSR to load data. Moreover, in this phase,  we exploit the designed VFEXP that executes the exponentiation of a \gls{simd} vector of 4 elements in XX cycles, while the baseline kernel performs the exp in software as described in Section XX, with a throughput of XX exp operation per cycle [or here we can mention the latency per each BF 16 exponentiation]. (( HERE MENTION THAT YOU ALSO ACCUMULATE FOR THE DEOMINATOR)
% Finally, we optimize the normalization step by computing the 1/sum outside the loop and we perform the scaling operation with a MUL oepration.
% Overall, these optimizations show XX advantages...[[advantages can be presented as #insns/output or similar metrics....]]


\subsection{Optimized Softmax Kernel}
\begin{table}[t]
\centering
\caption{Code Comparison of Baseline and Optimized Softmax Implementations}
\label{table:code_comparison}
\renewcommand{\baselinestretch}{1.0}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.0}

\begin{tabular}[t]{@{}p{0.4cm}p{3.4cm}p{4.2cm}@{}}
\hline
 & \textbf{Baseline} & \textbf{Optimized} \\
\hline
\rotatebox{90}{\parbox{1cm}{\centering Max}} &
\vspace{-3em}
\begin{lstlisting}
for (i = 0;i < N;i++){
  if (x[i] > max)
    max = x[i];
}
\end{lstlisting} &
\vspace{-3em}
\begin{lstlisting}
ssr ft0 read double;
frep.o %[n_frep],1;
vfmax.h ft3, ft3, ft0;
\end{lstlisting} \\[0pt]

\rotatebox{90}{\parbox{1cm}{\centering Exp}} &
\vspace{-3.5em}
\begin{lstlisting}
for (i = 0;i < N;i++){
  y[i]= exp(x[i]-max);
  sum += y[i];
}
\end{lstlisting} &
\vspace{-5em}
\begin{lstlisting}
ssr ft0 read double;
ssr ft1 write double;
frep.o %[n_frep],3;
vfsub.ah %[i],ft0,%[max];
vfexp.ah ft1,%[i];
vfadd.ah %[sum],%[sum],%[i];
\end{lstlisting} \\[0pt]

\rotatebox{90}{\parbox{1cm}{\centering Norm}} &
\vspace{-3.3em}
\begin{lstlisting}
for (i = 0;i < N;i++){
  y[i] /= sum;
}
\end{lstlisting} &
\vspace{-3.8em}
\begin{lstlisting}
ssr ft0 read double;
ssr ft1 write double;
frep.o %[n_frep],1;
vfmul.h ft1,%[1/sum],ft0;
\end{lstlisting} \\[0pt]

\end{tabular}
\end{table} 
We optimize the Softmax function to exploit the underlying ISA, including the designed instructions. Since the maximum value is required for the exponentiation step and must be computed by looping over each row of the resulting \( QK^T \) matrix, we construct the loop using the \texttt{FREP} instruction. As shown in \autoref{table:code_comparison}, targeting BF16 data and leveraging the core's 64-bit datapath, we utilize the \texttt{VFMAX} instruction in MAX step to balance computation and load costs - processing 4 \gls{simd} operations per 64-bit data load. To streamline data loads and keep the datapath fully utilized, we exploit the SSRs. 

The results are then forwarded to the exponentiation step (EXP), where we maintain a similar kernel structure using \texttt{FREP} and \texttt{SSR} for efficient data loading. In this phase, we leverage the \texttt{VFEXP} instruction, which performs the exponentiation of a \gls{simd} vector with 4 elements in 2 cycles. In contrast, the baseline kernel, described in Section 3.3, computes the exponentiation in software with a latency of 319 cycles per BF16 item. For each computed exponential, we also accumulate the sum using \texttt{VFADD} within the same \texttt{FREP SSR} loop. 

Finally, we optimize the normalization step (NORM) by calculating $1/\text{sum}$ outside the loop and performing a point-wise scaling operation with a \texttt{VFMUL} instruction. Overall, these optimizations achieve 2.15 instructions/output, significantly outperforming the baseline implementation, which requires 360 instructions/output, while also benefiting from loop unrolling advantages.






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\vspace{-0.85em}
\subsection{Optimized FlashAttention-2 Kernel}We optimize the partial Softmax part of the FlashAttention-2 kernel, which follows steps analogous to standard Softmax but performs them over multiple tiles. The optimization methods including \texttt{FREP}, \texttt{SSR} and \gls{simd} instructions (\texttt{VFEXP}, \texttt{VFMAX}, \texttt{VFSUB}, \texttt{VFMUL}) are employed in the same manner for the partial Softmax in FlashAttention-2 for partial MAX, EXP, and NORM. 


